Dissecting Latency in the Internet's Fiber Infrastructure

The recent publication of the `InterTubes' map of long-haul fiber-optic cables in the contiguous United States invites an exciting question: how much faster would the Internet be if routes were chosen to minimize latency? Previous measurement campaigns suggest the following rule of thumb for estimating Internet latency: multiply line-of-sight distance by 2.1, then divide by the speed of light in fiber. But a simple computation of shortest-path lengths through the conduits in the InterTubes map suggests that the conversion factor for all pairs of the 120 largest population centers in the U.S.\ could be reduced from 2.1 to 1.3, in the median, even using less than half of the links. To determine whether an overlay network could be used to provide shortest paths, and how well it would perform, we used the diverse server deployment of a CDN to measure latency across individual conduits. We were surprised to find, however, that latencies are sometimes much higher than would be predicted by conduit length alone. To understand why, we report findings from our analysis of network latency data from the backbones of two Tier-1 ISPs, two scientific and research networks, and the recently built fiber backbone of a CDN.

==> att.tex <==
\section{Latency Analysis for AT\&T}
\label{sec:att}
AT\&T publishes latencies between major cities in its  network on its Web site~\cite{att-latency}. 
Every 15 minutes the data is updated. We have collected this data between February 27, 2017 and April 7, 2017 by recording it every 30 minutes. The methodology and details of AT\&T's measurements in their backbone is explained in~\cite{att-methodology,att-ieee}.

\subsection{Latency Inflation in AT\&T's Network}

For each city pair in the published data, we computed the ratio of the AT\&T latency to the round-trip time for light to travel the line-of-sight distance between the city pair inside fiber. The blue line in figure~\ref{fig:att-latency}a shows the CDF of this ratio. We see that this ratio varies between $1.31$ and $4.0$ and the median value is $1.82$. The dotted purple line shows the same ratio when we use the shortest path length between the two cities (computed from the InterTubes dataset utilizing all the links marked as used/owned by AT\&T) as the baseline instead of the line-of-sight distance. Since we take the length of the fiber conduits into account, the purple line lies strictly to the left of the blue line, with minimum, median and maximum values being $1.00$,$1.33$ and $3.05$. 

The computation of the shortest paths revealed the existence of some links in AT\&T's backbone not included in the InterTubes dataset. This is because when we did this computation for the 259 city pairs  utilizing just AT\&T links according to the InterTubes dataset, we identified city pairs for which the published latency violated the speed-of-light constraint. This can only happen if there are links in AT\&T's backbone which do not exist in the InterTubes dataset, or even if the link is in the dataset, it is not marked as used/owned by AT\&T. For example, in the dataset there is a fiber conduit between Chicago and Indianapolis, with length $322.8$ km, but this conduit is not marked as used by AT\&T. Over this fiber conduit, the round-trip travel time of light is $3.16$ ms. However, the shortest path with AT\&T's links is found as the $927.86$ km long  \textit{Chicago-Springfield-St.Louis-Indianapolis} path, resulting in a lower bound of $9.1$ ms round-trip travel time. However, the minimum latency published by AT\&T is $5$ ms between Chicago and Indianapolis, illuminating the problem with the InterTubes dataset. Note that even if we assume the direct link between Chicago and Indianapolis is in AT\&T's backbone, resulting latency inflation would be $58\%$ which is more than what we would expect. We have identified 7 city pairs (out of 259 for which we have latency data) for which the shortest paths found using AT\&T's links in the InterTubes dataset result in speed-of-light violations based on the published RTTs.

The fact that some of AT\&T's links are missing is probably causing some inflation values reported above and plotted in figure~\ref{fig:att-latency}a to be lower than they really are. Missing links increase the shortest path length for some city pairs, lowering the computed inflation and masking the real one. That's why we probably see a minimum inflation of $1.00$ (since we also removed 7 city pairs with inflation values <1 implying speed-of-light violations). This explanation is also supported by the CDFs plotted in figure~\ref{fig:att-latency}b for the city pairs with a direct fiber conduit between them. 
For the corresponding purple line, the minimum, median and maximum of the inflation over $c$-latency is found as $1.14$,$1.47$ and $3.05$ respectively. Figure~\ref{fig:att-scatter} provides further proof of this, since some of the largest inflations are observed for city pairs with a direct link between them, and some very low inflations are between cities $5$ and $7$ hops away.

\begin{figure*}[t]
	\centering
	\subfigure[All City Pairs]{{\includegraphics[width=3.33in]{figures/att-vs-clatency.pdf} }}%
	\subfigure[City Pairs connected with a direct fiber conduit ]{{\includegraphics[width=3.33in]{figures/att-vs-clatency-direct.pdf} }}%
	\caption{Inflation in AT\&T's network}%
	\label{fig:att-latency}%
\end{figure*}

\begin{figure}
	\centering
	\includegraphics[width=3.33in]{figures/att-inflation-sp-vs-nhops-scatter.pdf}
	\caption{Latency inflation over shortest-path c-latency vs. number of hops in the shortest-path between each city pair}
	\label{fig:att-scatter}
\end{figure}


\subsection{Comparison of latencies in AT\&T's Network  and measurements using a large CDN}
In section~\ref{sec:cdn} we described the measurements we performed between the servers of a large CDN. 
The CDN uses AT\&T for network connectivity at multiple places and some of our measurements were between CDN servers both of which using AT\&T as the network provider. $16$ city pairs in AT\&T's latency data have a fiber conduit between them marked as used/owned by AT\&T in the InterTubes dataset(the left-most points in figure~\ref{fig:att-scatter}). Between $8$ of these cities we have measurements in the CDN data, with both endpoints getting network connectivity from AT\&T. For these city pairs, the comparison of the latencies published by AT\&T and performed by us between the CDN servers is presented in table~\ref{table:att-vs-cdn}. In general, latencies in the CDN data are slightly higher than observed in AT\&T data, except for Indianapolis and St. Louis pair. 

The slightly larger latencies in the CDN data can potentially be explained by two factors: 1- Our measurements between CDN servers were performed in $3-6$ hour intervals over a few days, with $~10$ measurements on average per city pair, whereas the AT\&T data covers roughly a 5-week period with data updated by AT\&T every 15 minutes; 2 - Each CDN server is selected using a $25$km radius from the conduit endpoint locations, resulting in a few extra hops (and distance) before routers in the core. Regardless, latencies observed in both networks are substantially higher than $c$-latency, except for Dallas Houston pair where minimum latency in AT\&T data is only slightly higher ($14\%$) than $c$-latency. For example, both latencies between Atlanta and Nashville are more than $2\times$ inflated in table~\ref{table:att-vs-cdn} and the AT\&T's published latency between Indianapolis and St. Louis is almost $3\times$ inflated over $c$-latency.

We shared this data with AT\&T engineers to get their opinion about what might cause these large inflations.
We received a comment about some of the link lengths in our data being somewhat short. We also learned that "depending on the transmission technology in use, dispersion compensation can increase the link latency by up to $17\%$". This happens because over large distances a single wave in fiber is dispersed into multiple colors traveling in different speeds, and extra spools of fiber are used at optical amplifiers to merge the signals traveling at different speeds. For example, a dispersion compensating fiber(DCF) system of length $1000$ km would require 12 amplifiers, each containing a small spool of DCF. Assuming that standard single-mode fiber is used, then the total length of the DCF would be about  170 km, so each of the optical amplifiers would have about 14 km of DCF.  Note that these are ball-park numbers, obtained through personal communication with an AT\&T engineer. Mentioned $17\%$ percent overhead due to DCF is consistent with the $15-25\%$ extra latency overhead due to DCF given in~\cite{bobrovs-dcf}. Even though DCF(extra fiber spools) might be a contributing factor,  $2-3\times$ inflation in the observed latencies over some links still requires an explanation. The most logical explanation would be the use of a significantly longer fiber route, which might or might not be captured in the InterTubes dataset; however this is not something we are able to verify yet.

\begin{table*}[t]
	\centering
	\begin{tabular}{llcccr}
		City 1 & City 2  & Conduit Length(km) & CDN Min. RTT(ms) & AT\&T Min. RTT(ms) & $c$-latency(ms)\\
		\hline
		Atlanta & Dallas & 1418.38 & 18.32 & 17 & 13.91 \\
		Atlanta & Nashville & 405.31 & 9.26 & 8 & 3.97 \\
		Dallas & Houston & 446.69 & 6.55 & 5 & 4.38 \\
		Dallas & New Orleans & 826.97 & 13.40 & 12 & 8.11 \\
		Houston & San Antonio & 379.80 & 5.28 & 5 & 3.72 \\
		Indianapolis & St. Louis & 434.21 & 7.35 & 13 & 4.26 \\
		Kansas City & St. Louis & 458.10 & 6.28 & 6 & 4.49 \\
		Nashville & St. Louis & 460.99 & 12.85 & 12 & 4.52
	\end{tabular}
	\caption{Comparison of  latencies of the CDN and AT\&T over fiber conduits in AT\&T's backbone}
	\label{table:att-vs-cdn}
\end{table*}

==> conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
The measurements we performed between CDN clusters and the latency data we obtained from a large ISP(AT\&T) exhibit much larger inflations over the speed-of-light along the fiber lengths than we anticipated. Here we discuss a few potential contributors of this outcome.

One obvious factor is the uncertainty we have in terms of the reliability of the InterTubes dataset we used. We have uncertainty not only in the endpoint locations of the fiber conduits but also in the provided link lengths. Despite the authors doing their best in collecting and verifying the link lengths, it seems the quality of the link lengths is probably not uniform. Some of these lengths are obtained from the ISPs owning the links and these are probably more accurate than the rest. For others, the authors calculated lengths based on the route it takes over the surface of the Earth by computing line-of-sight distances for each segment in the fiber route. The routes seem to be obtained by visually inspecting published maps, railroads and other right-of-ways which fiber conduits typically follow. It is possible that the link lengths that are shorter than their counterparts in ESnet or Internet2, and the lengths that are described as being "somewhat short" by the AT\&T engineers are obtained this way. However, it is very difficult to be certain about this without examining the routes themselves as there are often multiple fiber routes between same pairs of locations with markedly different lengths~\cite{riot-games}.

Another factor is the "hidden" sources of latency in the optical layer even in the case of accurate lengths based on fiber routes. Based on the transmission technology used inside the fiber, there might be additional spools due to dispersion compensation, increasing the distance the light needs to travel inside the fiber. Unfortunately the fibers owned/used by different ISPs are laid out in different times, and depending on the available transmission technology and the cost at the time, they may have very different characteristics. The only way to be certain about the actual lengths is by computing them based on tests in the physical layer. However, this is difficult to obtain in most cases. It is possible that some of the lengths in the InterTubes dataset (the ones obtained from published ISP data) are based on tests in the physical layer, but it is not possible to identify which.

Yet another factor is our use of traceroutes to obtain RTTs along the fiber conduits, with no visibility below IP layer. We did geolocate the routers in the traceroutes and try to understand which measurements followed routes along the intended conduit. Despite errors in geolocation, we were able to find measurements which showed with high likelihood the path along the fiber conduit was taken. However, for some of these measurements the RTTs are still higher than we expect and we cannot determine whether this is due to inaccurate link lengths or longer MPLS tunnels below the IP layer. 

It is encouraging to note that the RTTs we observed in ESnet are much closer to the physical limit imposed by speed-of-light. However, for these measurements we not only had very accurate link lengths obtained from tests in the physical layer, but also were able to verify that traceroutes followed the intended fiber conduits.

==> temp.tex <==
\subsection{Stretch of Shortest Fiber Paths}\label{sec:stretch}

Motivated by the observation that the fiber conduits are, in the median, only $20\%$ longer than geodesic distances, we examine how close shortest fiber path lenghts between arbitrary locations to the line-of-sight distance between them. 
% the following question: \stress{Is it possible to minimize the stretch between any two endpoints (from the InterTubes data set) by stitching together \stress{optimal} paths using the conduits?}
To answer this question, we compute the shortest fiber paths between all pairs of $273$ endpoints in the data set and divide the length of each fiber path with the corresponding \newterm{geodesic} distance to calculate its stretch.
We find that it is possible to obtain a stretch of $1.32$ in the median (and $1.86$ in the 95-th percentile) for the shortest fiber paths between all pairs of $273$ endpoints in the data set.
% These stretch values reflect that latency observed by traffic is only $30\%$ larger than \frtt---the theoretical limit on latency achievable in optical fiber, equal to two-thirds the speed of light in vacuum---using all known fiber conduits in the US.
Implicit in the analysis is the assumption that each fiber endpoint contributes \stress{equally} to the traffic. If we, however, use a gravity model for traffic (i.e., traffic between any two of the $273$ endpoints is proportional to the product of the population at the endpoints), the stretch values reduce further to a value of $1.26$ in the median and $1.56$ in the 95-th percentile.\footnote{We use population estimates from the 2013 census data.}

% We computed the shortest fiber paths between all pairs of $273$ endpoints in the InterTubes dataset.
% Dividing the shortest path length by the geodesic distance between the conduit endpoints we obtain the \textit{stretch} for each endpoint pair. We see that median and $95$-th percentile stretch are $1.32$ and $1.86$ respectively. These values reflect the achievable inflation beyond $c$-latency \fix{f-latency? used without definition} on a network using all available (known) fiber in the US, assuming each fiber end-point contributes equally to the traffic. When a gravity model of traffic is used (\ie traffic between two locations is proportional to the product of their populations), median and $95$-th percentile values are $1.26$ and $1.56$.

\begin{figure*}[t]
	\centering
	\subfigure[CDF of path stretch]{\label{fig:path-stretch-cmp}
	    {\includegraphics[width=3.3in]{figures/stretch-cdf.pdf}}}
	%\subfigure[CDF of path lengths (hop count)]{\label{fig:cdf-num-hops}
	    %{\includegraphics[width=2.2in]{figures/nhops-cdf.pdf}}}
	\subfigure[Stretch for different path lengths]{\label{fig:cdf-hops-stretch}
	    {\includegraphics[width=3.3in]{figures/stretch-vs-nhops.pdf}}}
	
	\caption{Results of all-pairs-shortest-path computation}%
	\label{fig:path-stretch}%
\end{figure*}

We repeated the same analysis, separately, for each ISP in the data set. 
% Table~\ref{table-isp-size} shows the median and $95$-th percentile stretch values for the $9$ largest ISPs, each of which has long-haul links connecting over $100$ locations.
% The values in Table~\ref{table-isp-size} are not directly comparable to the stretch values for the entire set of $273$ locations: no single ISP covers all endpoints; even the largest ISP covers only $248$ of the $273$ endpoints\footnote{We use the list of ISPs and their links as reported in the InterTubes data set, ignoring mergers and acquisitions since then, such as CenturyLink's acquisition of Level3. Obviously with such mergers ISPs increase their geographic footprint and can find direct, low-latency paths between more locations.}.
EarthLink and Level3\footnote{Now part of CenturyLink.} have the largest number of fiber conduits in their backbones, each being associated with nearly $85\%$ of all the conduits provided in the data set; the stretch values for these two networks are very close to the corresponding values for the entire data set.
Networks with smaller number of fiber conduits, in contrast, have relatively large stretch values.
% For networks with smaller number of fiber conduits, both median and $95$-th percentile stretch values are larger. 

% \begin{table}[h]
% 	\centering
% 	\begin{tabular}{r|cc}
% 	\toprule
% 	\textbf{ISP} & \textbf{Median} & \textbf{95$^{th}$\%} \\
% 	\midrule
%         EarthLink & 1.35 & 1.83 \\
%         Level3 & 1.36 & 1.83 \\
%         Comcast & 1.48 & 2.11 \\
%         CenturyLink & 1.55 & 3.37 \\
%         TWC* & 1.48 & 2.03 \\
%         Verizon & 1.54 & 2.16 \\
%         ATT & 1.43 & 2.66 \\
%         Sprint* & 1.75 & 5.47 \\
%         HurricaneElectric* & 1.45 & 2.67 
% 	\end{tabular}
% 	\caption{Stretch values computed separately for a few ISPs for shortest fiber paths using only links of the given ISP.}
% 	\label{table-isp-size}
% \end{table}
All pairs shortest paths computations for individual ISPs revealed that for $8$ ISPs (out of $20$) the network consisting of all the links marked with that ISP (in the InterTubes data set) is disconnected. 
% The asterisk (*) next to some of the ISP names in Table~\ref{table-isp-size} denotes that the network consisting of all the links marked with that ISP (in the InterTubes data set) is \stress{not} connected. Consequently, we computed the stretch for such ISPs by considering only the pairs of connected endpoints.
% Considering only a subset of the endpoints for the stretch computation might be a reason for the high stretch values of some of these ISPs.
%\PENDING{What are we trying to convey?}
This can be due to either some fiber conduits not being captured in the dataset or some existing conduits in the dataset are used by more ISPs than listed. Advertised round-trip times between major locations in AT\&T's network~\cite{att-latency} also reveal that not all links of a network's backbone are captured in the data set, since published RTTs for some city pairs violate speed-of-light constraints based on AT\&T's links reported in the InterTubes dataset.
% \PENDING{Why would these publicly shared RTTs reveal anything about the InterTubes data set? We have to be clear on how it helps.}
% \PENDING{Not sure how to end this paragraph}

% Most likely, some of the listed ISPs have additional long-haul links in their backbones, either due to a particular link itself or the information that an ISP being on that link not captured in the InterTubes dataset.
% In Table~\ref{table-isp-size} we appended an $*$ to some ISP names, which indicate that the network consisting of all the links marked with that ISP is not connected. The stretch computations were done over pairs of connected endpoints for these ISPs. This might be one reason for higher stretch values for some of the ISPs. Moreover, published RTTs between major locations in AT\&T's network proves that there are additional links in AT\&T network as we discuss in section~\ref{sec:att}. Regardless, since a recent measurement study has reported end-to-end latencies over default routes between well-connected locations as $3$-$4\times$ inflated over $c$-latency~\cite{soslow-pam17}, being able to aggregate and utilize the entirety of this fiber infrastructure could reduce latencies by as much as $50\%$. Moreover, some of the $273$ fiber conduit endpoints are in places with a very small population, and ignoring these places might improve the stretch values.

% Lastly, some of the $273$ fiber conduit endpoints are in locations with a very small population \PENDING{numbers?}.
% We may, initially, ignore such places in the design, but connect such less populous places to the network, later, incrementally, to keep the stretch values low.
% To examine such an incremental design, we repeated the stretch analysis between $248$ endpoints that had a population size of at least $\num{20000}$ or more; constraining by high population only removed $25$ endpoints of the total $273$.
% The stretch values for this design, in Figure~\ref{fig:path-stretch-cmp} shrink to $1.27$ (from $1.32$) in the median and to $1.76$ (from $1.86$) in the 95-th percentile. \PENDING{How do we justify a drop of 4-5\% in stretch when ignoring 9\% of endpoints?}
% Further, weighting the endpoints by traffic using a gravity model shrinks the stretch to $1.20$ and $1.54$ in the median and 95-th percentile, respectively; Figure~\ref{fig:path-stretch} shows that the dashed line corresponding to the gravity model lies strictly to the left of the unweighted case.

Some of the $273$ fiber conduit endpoints are in places with a very small population, e.g. a few thousand, and ignoring these places might improve the stretch values.
To examine this, we repeated the same computation between endpoint locations with population at least $20,000$.
In this case, all-pairs shortest path computation for the remaining $248$ cities results in median and $95$-th percentile stretch values $1.27$ and $1.76$ respectively. Using the gravity model, stretch values improve further and median and $95$-th percentile stretch are found as $1.20$ and $1.54$ respectively. Figure~\ref{fig:path-stretch}a shows the CDF of stretch with these two traffic models and we see that the dashed line for the gravity model lies strictly to the left of unweighted case. 

% One might conjecture, based on the CDF of stretch in Figure~\ref{fig:path-stretch-cmp} for the unweighted case, that the long tail (i.e., beyond the 95-th percentile) are caused by long circuitous paths formed from several conduits. The distribution of the number of hops between each pair of endpoints, where each hop is a fiber endpoint in a different city, shows the median and 95-th percentile values are $7$ and $14$, respectively.
% \PENDING{Do large number of hops imply a higher stretch?}
% Figure~\ref{fig:path-stretch}c shows the CDFs of stretch for three intervals for the number of hops between the pairs of endpoints: less than $3$, between $3$ and $7$, and more than $7$.
% For the small values of stretch, larger number of hops correlate with higher stretch. \PENDING{Small values?}
% However, the curves meet around $60$-th percentile, and for the higher stretch values in the tail, we see the opposite. Examining a few cases we observe this is potentially due to some paths having a large number of intermediate cities along a relatively straight path, with little impact on stretch.
% \PENDING{Needs more polish; we could get rid of Fig.2b}

Even though the median and even the $95$-th percentile stretch values are promising, it is interesting to examine the relationship between stretch and the number of hops for each city pair. One might conjecture that higher stretch values in the tail are caused by long circuitous paths.
The distribution of the number of hops between each pair of endpoints, where each hop is a fiber endpoint in a different city, shows the median and $95$-th percentile values are $7$ and $14$, respectively.
Figure~\ref{fig:cdf-hops-stretch} shows that paths with just one intermediate hop have stretch values in a very wide range, and the worst stretch values are for the paths with length between $2$ and $7$ hops. As the path length increases above $10$, observed minimum stretch values increase but the largest stretch values stay far below the worst stretch values for the shorter paths. Examining a few cases, we observed that this is potentially due to some paths having a large number of intermediate cities along a relatively straight path, with little impact on stretch.    
% Figure~\ref{fig:path-stretch}b shows the CDF of the number of hops between each pair of endpoints. We observe that the median and the $95$-th percentile path lengths are $7$ and $14$ hops respectively.
% Note that each hop in this analysis is a fiber endpoint in a different city but our analysis here just focuses on the impact of fiber paths passing through these intermediate locations on the total length of the fiber path. 
% Long circuits can be established between two distant endpoints while avoiding optical switching and routing at the intermediate locations, as we briefly touch on section~\ref{sec:fiber-latency}. Figure~\ref{fig:path-stretch}c shows the 
% CDFs of stretch for three intervals for the number of hops between the pairs of endpoints: less than $3$, between $3$ and $7$, and more than $7$. For the small values of stretch, larger number of hops correlate with higher stretch. However, the curves meet around $60$-th percentile, and for the higher stretch values in the tail, we see the opposite. Examining a few cases we observe this is potentially due to some paths having a large number of intermediate cities along a relatively straight path, with little impact on stretch.

Overall we observe that the stretch values are very promising.
% The bottom line is that conduits are close to line of sight with a median stretch of only $1.2$. We can string together such conduits to connect all $273$ endpoints (in the InterTubes data set) with a stretch of $1.32$ in the median. 
It is, however, not realistic to assume that we can use \stress{all} the available fiber infrastructure in US.  
%
% Nevertheless, recall that some of the endpoints used in the above analyses are not \stress{ideal} locations to connect, and we demonstrated that the stretch can be lowered further through a more judicious choice of endpoints.
% Next, we delve into the details of the choice of endpoints and identification of a critical set of fiber conduits to connect these endpoints while incurring only a small stretch.
%
% Overall we observe that the stretch values are very promising. However it is not realistic to assume we can use all the available fiber in US. 
Moreover, some of the endpoints we used in the above analysis are not ideal locations to target. In the next section, we target a smaller set of large population centers while identifying a critical set of fiber conduits to connect these large population centers while keeping the increase in stretch as small as possible.

